Real-Time Facial Segmentation and Performance Capture from RGB Input

We introduce the concept of unconstrained real-time 3D facial performance capture through explicit semantic segmentation in the RGB input. To ensure robustness, cutting edge supervised learning approaches rely on large training datasets of face images captured in the wild. While impressive tracking quality has been demonstrated for faces that are largely visible, any occlusion due to hair, accessories, or hand-to-face gestures would result in significant visual artifacts and loss of tracking accuracy. The modeling of occlusions has been mostly avoided due to its immense space of appearance variability. To address this curse of high dimensionality, we perform tracking in unconstrained images assuming non-face regions can be fully masked out. Along with recent breakthroughs in deep learning, we demonstrate that pixel-level facial segmentation is possible in real-time by repurposing convolutional neural networks designed originally for general semantic segmentation. We develop an efficient architecture based on a two-stream deconvolution network with complementary characteristics, and introduce carefully designed training samples and data augmentation strategies for improved segmentation accuracy and robustness. We adopt a state-of-the-art regression-based facial tracking framework with segmented face images as training, and demonstrate accurate and uninterrupted facial performance capture in the presence of extreme occlusion and even side views. Furthermore, the resulting segmentation can be directly used to composite partial 3D face models on the input images and enable seamless facial manipulation tasks, such as virtual make-up or face replacement.

==> problem_statement.tex <==
\section{Problem Statement}\label{sec:problem}

\begin{figure*}[t!]
 \centering
\includegraphics[width=\textwidth]{images/overview/overview}
\caption{Here is an overview of our system
 \label{fig:overview}}
\end{figure*}


\begin{figure}[h!]
 \centering
\includegraphics[width=\columnwidth]{images/overview/system.pdf}
\caption{Capture Setting.
 \label{fig:system}}
\end{figure}


% go through idea here, need to be short, concise, beautiful

* We would like to state the idea to solve unconstrained facial capturing in a more general way, as the problem share common setting with other applications like detection, tracking etc.

Generally, facial applications including detection, tracking, and landmark alignment require algorithms to not only predict facial features e.g. shape positions or expression, but also have a sophisticated system to robustly handle the variation of appearance under unconstrained situation.

In fact, since shape and motion of face can be reliably determined using very few parameters, most of the variation of input comes from objects non-directly related to the face itself, as known as background or occlusion depending on their relative position towards the face.
Since the appearance of such regions is independent with and cannot provide extra guidance to the face, improving facial capture performance by first segmenting and removing unrelated region becomes an intuitive idea.

While the idea itself is simple, the idea beneath this optimization should draw more concern as it reveals a more general methodology and can be applied to improve large amount of existing algorithm handling performance capturing allowing wild environment with potential occlusion.

To recover interesting information of the face, considered as an specific object in the scene of the input image, the variance of all other objects, including light source, camera or other objects obviously cannot help, and should not influence the process.
Although some environment factors e.g. lighting or motion of camera will affect the appearance of one's face, and they are coupled with the parameter of face in the input image within the region of interest, they can be described using simple models and are already well examined (white balance, debluring, denoising etc).

The main challenge lays on the existence of other objects and their highly variant appearance, which by principle cannot be modeled (because arbitrary things can exist at the background).
And as most of occluding objects are not transparent, the regions occupied by them cannot provide any further information to the face.
Note that occluded regions are different from image noise because of inaccurate measurement, e.g. motion blur or exposure noise.
Noisy observation are derived from the ground truth, thus information can still be recovered or reliably estimated given the model of the occurrence of noise.
Occlusions, however, is independent from the desired information.

Therefore, reliably masking out such regions will greatly reduce the variance of input data, without losing any potential information. Existing methods can hence benefit from a much simpler range of input. Since the appearance of background and occlusion are unpredictable, this is also the only possible way to minimize the influence brought by change of such regions.

In fact, with reliable face segmentation, accuracies of existing methods~\cite{cao2014displaced} can be improved as shown in Sec~\ref{sec:result}.
This indicates that although such methods claim to handle variation including occlusion, the intrinsic process of it didn't succeed in eliminating the effect from unrelated objects better than a separate segmentation step does.

Although the segmentation between the face region and unrelated ones contains more indeterminism, a rough region estimation can be obtained quickly with modern GPU and the concept of convolutional neural network in image processing. With further efficient and deterministic (non-learning) refinement we show that an accurate face segmentation in real-time is possible, making this step of image processing ``cost nothing'' and has its potential to become a standard data preprocessing step before any facial capture technique.

% hardness of this problem
%* The segmentation and face capture is a chick and egg problem.
%While the capture problem is more concrete and the segmentation seems to be harder to be solved, its wild application draws people's attention and there are works in the computer vision attacking general image segmentation task quite successfully.
%The segmentation challenge such as in ILSVRC focus on general segmentation between different categories of objects in wild, however to segment only the facial part our of the whole human haven't been studied thoroughly yet.






% here are words from Shunsuke, need reorganize
%Regression has been widely adopted by facial applications such as detection, tracking, and landmark alignment. Given training data, regression-based approaches learn a direct mapping function $\Phi$ from image appearance $\F$ to the target output $\P$ (e.g., landmark locations, 3D shape, or blend shape coefficients). In the unconstrained situation, however, the input image appearance may contain non-face objects front or behind faces. Since arbitrary objects can be present in the image, occluding objects and background can be regarded as noise. Recently researchers have attempted to improve the robustness of regression by cascading weak regressors based on large training data, it is still difficult to model occlusion due to its immense space of appearance variability. Thus, instead, we propose to reduce appearance variability in the images by masking out non-face regions as if the input image only contains a face in both training and inference processes. In this paper, by applying it to facial performance capture, we demonstrate this observation drastically improves the robustness In Sec~\ref{sec:system}, we explain the overview of our system architecture enabling high-fidelity face/non-face segmentation and robust facial performance capture in realtime. We will describe how we obtain segmentation mask in order to achieve robust cascade regression (Sec~\ref{sec:probmap}) and how we incorporate resulting segmentation into regression-based facial tracking (Sec~\ref{sec:tracking}). Sec~\ref{sec:result} demonstrait that our method outperform other state-of-the art methods and achives robust segmentation and face tracking in the challenging cases such as occlusion and large rotation.
%\Shun{TODO: rephrase noise in this section}
